Scientific Talent Leaks Out of Funding Gaps

We study how delays in NIH grant funding affect the career outcomes of research personnel. Using comprehensive earnings and tax records linked to university transaction data along with a difference-in-differences design, we find that a funding interruption of more than 30 days has a substantial effect on job placements for personnel who work in labs with a single NIH R01 research grant, including a 3 percentage point (40%) increase in the probability of not working in the US. Incorporating information from the full 2020 Decennial Census and data on publications, we find that about half of those induced into nonemployment appear to permanently leave the US and are 90% less likely to publish in a given year, with even larger impacts for trainees (postdocs and graduate students). Among personnel who continue to work in the US, we find that interrupted personnel earn 20% less than their continuously-funded peers, with the largest declines concentrated among trainees and other non-faculty personnel (such as staff and undergraduates). Overall, funding delays account for about 5% of US nonemployment in our data, indicating that they have a meaningful effect on the scientific labor force at the national level.

==> tables/amendments-tab.tex <==

\begin{tabular}{cc}
\hline\hline
\vspace{-12pt} \\
          & Interruption \\
          & (1) \\
\midrule
Amendments & 0.12*** \\
           & (0.01) \\
\vspace{-12pt} \\
\hline\hline
\end{tabular}


%\begin{tabular}{ccc}
%\toprule
%Variable & Estimate & P-value\\
%\midrule
%No. of amendments & \makecell[c]{0.12***\\0.01} & 0\\
%\bottomrule
%\end{tabular}


==> tables/demobalance.tex <==
\begin{tabular}[t]{lccc}
\toprule
 & Continuously Funded  & \hspace{1cm} & Interrupted \\
\midrule
Lab \% Female & 0.4583 && 0.4352 \\
 & (0.2871) && (0.2954) \\
Lab \% Asian & 0.2704 && 0.292 \\
 & (0.2776) && (0.3193) \\
Lab \% Black & 0.02252 && 0.03342 \\
 & (0.08274) && (0.1116) \\
Lab \% White & 0.674 && 0.6489 \\
 & (0.2957) && (0.3229) \\
Lab \% Hispanic & 0.04725 && 0.03959 \\
 & (0.1217) && (0.122) \\
Lab \% US-Born & 0.5596 && 0.5744 \\
 & (0.3248) && (0.3388) \\
\bottomrule
\multicolumn{4}{p{0.65\linewidth}}{ \small This table shows the percent of each single-R01 lab that has particular demographic characteristics at T-1.}\\
\end{tabular}

==> tables/neweinold.tex <==
\begin{tabular}[t]{lll}
\toprule
EIN type & Estimate & SE\\
\midrule
New University & 0.03695** & (0.01782)\\
New Non-University & -0.02181 & (0.01889)\\
\bottomrule
\multicolumn{3}{l}{\textsuperscript{} Table 2: This table shows aggregated estimates}\\
\multicolumn{3}{l}{of the average treatment effects (ATTs) in our}\\
\multicolumn{3}{l}{single-R01 sample of an interruption on the}\\
\multicolumn{3}{l}{count of new university and non-university}\\
\multicolumn{3}{l}{EINs that pay wages to a person in a given}\\
\multicolumn{3}{l}{year. The effects are aggregated over the 5}\\
\multicolumn{3}{l}{years after the expiration of a lab’s grant.}\\
\multicolumn{3}{l}{The estimates are obtained using a modified}\\
\multicolumn{3}{l}{Calloway-Sant’Anna (2020) estimator. Standard}\\
\multicolumn{3}{l}{errors are bootstrapped and clustered at the}\\
\multicolumn{3}{l}{interrupted R01 level.}\\
\end{tabular}

==> tables/noadmincensus.tex <==
\begin{tabular}[t]{lccc}
\toprule
& In 2020 Census & \hspace{1cm} & Not In 2020 Census \\
\midrule
 &  0.0146  &&  0.0156**\\
 & (0.0096) && (0.0067)\\
\bottomrule
\multicolumn{4}{p{0.65\linewidth}}{ \small This table shows aggregated estimates of the average treatment effects (ATTs) in our single-R01 sample of an interruption on the not being found in the administrative data, split by whether or not a person is observed in the 2020 Decennial Census. The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.}\\
\end{tabular}

==> tables/noadmincensus_copy.tex <==

\begin{tabular}[c]{lccc}
\toprule
Subsample \hspace{3cm} &  In 2020 Census & \hspace{1cm} & Not In 2020 Census\\
&  Absent From Tax Data && Absent From Tax Data\\
\midrule

All &  0.0146  &&  0.0156**\\
    & (0.0096) && (0.0067)\\

\addlinespace
\midrule
\addlinespace
Foreign-born &  -0.00887 && 0.0282 \\
             & (0.0127) && (0.0184) \\

\addlinespace
US-born &  0.0262** &&  0.0106** \\
        & (0.0114) && (0.0052) \\
\addlinespace
\midrule
\addlinespace

Faculty & 0.0061 && -0.00208 \\
        & (0.0141) && (0.0177) \\
\addlinespace
Postdoc/Grad & 0.0193 && 0.0432** \\
             & (0.0178) && (0.0177)\\
\addlinespace
Other & 0.015  && 0.0114 \\
      & (0.0126) && (0.0083)\\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\small
\item [] This table shows aggregated estimates of the average treatment effects (ATTs) in our single-R01 sample of an interruption on the not being found in the administrative data, split by whether or not a person is observed in the 2020 Decennial Census.  For each group, the coefficients should sum to the overall estimate of not finding people in the administrative data. The first two rows are for all people in  single-R01 labs, and the ones below it are for different sub-groups of these labs.  The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.
\end{tablenotes}

==> tables/noadmindataold.tex <==
\begin{tabular}[t]{llllll}
\toprule
Subsample & \# R01 & Not in admin data & In 2020 Census & Estimate & SE\\
\midrule
All & Single & Yes & Yes & 0.01465 & (0.009575)\\
All & Single & Yes & No & 0.01559** & (0.006694)\\
Foreign-born & Single & Yes & Yes & -0.008865 & (0.01274)\\
Foreign-born & Single & Yes & No & 0.0282 & (0.01844)\\
US-born & Single & Yes & Yes & 0.0262** & (0.01138)\\
\addlinespace
US-born & Single & Yes & No & 0.01063** & (0.00519)\\
Faculty & Single & Yes & Yes & 0.006097 & (0.01414)\\
Faculty & Single & Yes & No & -0.002078 & (0.01766)\\
Postdoc/Grad & Single & Yes & Yes & 0.01925 & (0.01776)\\
Postdoc/Grad & Single & Yes & No & 0.04315** & (0.01773)\\
\addlinespace
Other & Single & Yes & Yes & 0.01498 & (0.01257)\\
Other & Single & Yes & No & 0.01143 & (0.008268)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\small
\item [] This table shows aggregated estimates of the average treatment effects (ATTs) in our single-R01 sample of an interruption on the not being found in the administrative data, split by whether or not a person is observed in the 2020 Decennial Census.  For each group, the coefficients should sum to the overall estimate of not finding people in the administrative data. The first two rows are for all people in  single-R01 labs, and the ones below it are for different sub-groups of these labs.  The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.
\end{tablenotes}

==> tables/ownunivold.tex <==



\begin{tabular}[t]{llrrrr}
\toprule
Subsample & At Original (UMETRICS) University & At New University\\
Subsample & At Original University & At New University\\
\midrule
All & -0.02112  & 0.02404 \\
& (0.02153) & (0.01818) \\
All & At New University  & -0.0115928 & 0.0596728\\
US-born & At Original University & -0.03898 & 0.02495 & -0.0878820 & 0.0099220\\
US-born & At New University & 0.03245 & 0.02280 & -0.0122380 & 0.0771380\\
Foreign-born & At Original University & 0.01766 & 0.02812 & -0.0374552 & 0.0727752\\
\addlinespace
Foreign-born & At New University & 0.00705 & 0.02237 & -0.0367952 & 0.0508952\\
\bottomrule
\end{tabular}
\begin{tablenotes} [flushleft]
\small
\item [] This table shows aggregated estimates of the average treatment effects (ATTs) of in our single-R01 sample of an interruption on the probability of being at a person's original UMETRICS university and of being at any other university. The coefficients should sum to the main estimate of probability of being paid by a university. The first two rows are for all single-R01 employees, while the next two are for foreign-born employees, and the last two for US-born employees.The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.
\end{tablenotes}

==> tables/pubnoadmin-tab.tex <==

\begin{tabular}{lccc}
\toprule
& Publishing & \hspace{1cm} & Not Publishing\\
\midrule
& \makecell[c]{0.004\\(0.006)} && \makecell[c]{0.026***\\(0.009)}\\
\bottomrule
\end{tabular}


==> tables/pubnoadmin-tab_copy.tex <==
\begin{tabular}{lcc}
\toprule
Subsample & Publishing & Not Publishing\\
\midrule
All & \makecell[c]{0.004\\(0.006)} & \makecell[c]{0.026***\\(0.009)}\\
\midrule
US-born & \makecell[c]{-0.007\\(0.011)} & \makecell[c]{0.025\\(0.018)}\\
Foreign-born & \makecell[c]{0.011*\\(0.006)} & \makecell[c]{0.025***\\(0.010)}\\
\midrule
Faculty & \makecell[c]{0.010\\(0.014)} & \makecell[c]{-0.004\\(0.012)}\\
Postdoc/Grad & \makecell[c]{0.003\\(0.013)} & \makecell[c]{0.059***\\(0.021)}\\
\addlinespace
Others & \makecell[c]{0.007\\(0.007)} & \makecell[c]{0.020*\\(0.012)}\\
\bottomrule
\end{tabular}


==> tables/pubnoadmin.tex <==
% \begin{tabular}[c]{lccc}
% \toprule
% Subsample \hspace{3cm} &  Publishing & \hspace{1cm} & Not Publishing \\
% \midrule
% All & 0.0259*** && 0.0045 \\
%     & (0.00946) && (0.0059)\\
% \addlinespace
% \midrule
% \addlinespace
% Foreign-born & 0.0247 && -0.0066 \\
%              & (0.0184) && (0.0114)\\
% \addlinespace
% US-born  & 0.0253*** && 0.011* \\
%          & (0.00960) && (0.0059)\\
% \bottomrule
% \end{tabular}

\begin{tabular}[c]{lccc}
\toprule
Subsample & Publishing & & Not Publishing \\
\midrule
All & 0.0259*** & & 0.0045 \\
    & (0.00946) & & (0.0059)\\
\addlinespace
\midrule
Foreign-born & 0.0247 & & -0.0066 \\
             & (0.0184) & & (0.0114)\\
\addlinespace
US-born & 0.0253*** & & 0.011* \\
        & (0.00960) & & (0.0059)\\
\addlinespace
\midrule
\addlinespace
Faculty & 0.01008 & & -0.003775 \\
        & (0.0138) & & (0.01237)\\
\addlinespace
Postdoc/Grad & 0.00257 & & 0.05868*** \\
             & (0.01324) & & (0.02096)\\
\addlinespace
Others & 0.006563 & & 0.02032* \\
       & (0.007167) & & (0.01233)\\
\bottomrule
\end{tabular}

\begin{tablenotes}[flushleft]
\small
\item [] This table shows aggregated estimates of the average treatment effects (ATTs) in our single-R01 sample of an interruption on the not being found in the administrative data, split by whether or not a person is observed with a publication in MEDLINE.  For each group, the coefficients should sum to the overall estimate of not finding people in the administrative data. The first two rows are for all people in  single-R01 labs, and the next four split the lab into foreign- and US-born.  The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.
\end{tablenotes}

==> tables/pubnoadmincensusold.tex <==

\begin{tabular}[t]{llllll}
\toprule
Subsample & Not in admin data & Published & In 2020 Census & Estimate & SE\\
\midrule
Foreign-born & Yes & No & No & 0.0357** & (0.01725)\\
Foreign-born & Yes & No & Yes & -0.00977 & (0.01159)\\
Foreign-born & Yes & Yes & No & -0.007738 & (0.01156)\\
Foreign-born & Yes & Yes & Yes & 0.0009497 & (0.006306)\\
US-born & Yes & No & No & 0.008823* & (0.005007)\\
\addlinespace
US-born & Yes & No & Yes & 0.01815** & (0.008856)\\
US-born & Yes & Yes & No & 0.003393 & (0.004069)\\
US-born & Yes & Yes & Yes & 0.009127 & (0.005595)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\small
\item [] This table shows aggregated estimates of the average treatment effects (ATTs) in our single-R01 sample of an interruption on the not being found in the administrative data, split by two things: whether or not a person is observed with a publication in MEDLINE, and whether or not a person is observed in the 2020 Decennial Census.  For each group, the coefficients should sum to the overall estimate of not finding people in the administrative data. The first four rows are for all foreign-born people in single-R01 labs. The second four are for US-born people in single-R01 labs.  The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.
\end{tablenotes}

==> tables/pubnoadminold.tex <==

\begin{tabular}[t]{lllll}
\toprule
Subsample & Not in admin data & Published & Estimate & SE\\
\midrule
All & Yes & No & 0.02586*** & (0.009458)\\
All & Yes & Yes & 0.004483 & (0.005851)\\
Foreign-born & Yes & No & 0.02472 & (0.01844)\\
Foreign-born & Yes & Yes & -0.006551 & (0.01144)\\
US-born & Yes & No & 0.02525*** & (0.009597)\\
\addlinespace
US-born & Yes & Yes & 0.011* & (0.005925)\\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\small
\item [] This table shows aggregated estimates of the average treatment effects (ATTs) in our single-R01 sample of an interruption on the not being found in the administrative data, split by whether or not a person is observed with a publication in MEDLINE.  For each group, the coefficients should sum to the overall estimate of not finding people in the administrative data. The first two rows are for all people in  single-R01 labs, and the next four split the lab into foreign- and US-born.  The effects are aggregated over the 5 years after the expiration of a lab’s grant. The estimates are obtained using a modified \cite{callaway2020dd} estimator. Standard errors are bootstrapped and clustered at the interrupted R01 level.
\end{tablenotes}

==> tables/regressions.tex <==


\begin{tabular}{lccccccccccccccccccc} \hline\hline
& (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\
\hline
\hline
\\
\\
\textbf{Panel A: Multiple-R01 Labs} \\
\hline
& Personnel & R01s & Obs. & Univ.& Industry & No Admin. & UM Univ. & Non-UM Univ. & IHS Earnings\\
\hline
\\
\hspace{3mm}Full Sample                         & 13,500 & 1,200 & 229,000 & 0.005576 & 0.003727 & -0.009303 & 0.000309 & 0.001882 & 0.04929  \\
                                                & & & & (0.01325) & (0.01009) & (0.008569) & (0.01653) & (0.01059) & (0.0965) \\
                                                & & & & \{0.9137, 0.5750\} & \{0.0356, 0.2688\} & \{0.0507, 0.1562\} & \{, \} & \{, \} &  \\
                                                &  & &  & 1.65\% & 1.60\% & -8.82\% &  & & \\
\hline
\\
\\
\textbf{Panel A: Single-R01 Labs} \\
\hline
& Personnel & R01s & Obs. & Univ.& Industry & No Admin. & UM Univ. & Non-UM Univ. & IHS Earnings\\
\hline
\\
\hspace{3mm}Full Sample                            & 4,200 & 600 & 61,500 & -0.02104 & -0.009197 & 0.03024*** & -0.02112 & 0.02404 & -0.5228***  \\
                                                   &  & &  & (0.01843) & (0.0147) & (0.01168) & (0.02153) & (0.01818) & (0.1373) \\
                                                   &  & &  & \{0.9101, 0.6023\} & \{0.048, 0.2751\} & \{0.0419, 0.1226\} & \{0.8905, 0.4287\} & \{0.08685, 0.2046\} & \\
                                                   &  & &  & -6.84\% & -4.05\% & 37.5\% & -4.57\% & 20.4\% & \\
\\
\hspace{3mm}Faculty                                & 900 & 500 & 14,000 & -0.02134 & 0.02158 & 0.00302 & -0.04082** & 0.01098 & -0.1377  \\ 
                                                   &  & &  & (0.01778) & (0.01503) & (0.01523) & (0.02021) & (0.02091) & (0.1556) \\
                                                   &  & &  & \{0.9741, 0.8957\} & \{0.01773, 0.06082\} & \{0.008174, 0.04348\} & \{0.9659, 0.8232\} & \{0.09537, 0.1478\} & \\
                                                   &  & &  & -27.2\% & 50.1\% & 8.55\% & 28.6\% & 20.9\% & \\
\\
\hspace{3mm}Post-Doc/Grad Student                  & 1,300 & 400 & 18,500 & -0.05373* & -0.007316 & 0.06104*** & -0.07751** & 0.06125 & -0.7426***  \\
                                                   &  & &  & (0.03104) & (0.02404) & (0.02353) & (0.03307) & (0.03926) & (0.2772) \\
                                                   &  & &  & \{0.892, 0.5434\} & \{0.04821, 0.2981\} & \{0.05979, 0.1585\} & \{0.864, 0.266\} & \{0.108, 0.3151\} & \\
                                                   &  & &  & 15.4\% & -2.93\% & 61.8\% & -13.0\% & 29.6\% & \\
\\
\hspace{3mm}Post-Doc                               & 550 & 250 & 7,500 & -0.00903 & -0.07023*** & 0.07513* &  &  & -0.8227  \\
                                                   &  & &  & (0.04466) & (0.02607) & (0.04359) &  &  & (0.5213) \\
                                                   &  & &  & \{0.885, 0.523\} & \{0.035, 0.25\} & \{0.08, 0.227\} & \{0.85, 0.222\} & \{0.127, 0.319\} & \\
                                                   &  & &  & -2.49\% & -32.7\% & 51.1\% &  & & \\
\\
\hspace{3mm}Grad Student                           & 750 & 300 & 11,000 & -0.08853** & 0.03158 & 0.05865*** &  &  & -0.7494***  \\
                                                   &  & &  & (0.038) & (0.02955) & (0.02072) &  &  & (0.2505) \\
                                                   &  & &  & \{0.897, 0.557\} & \{0.057, 0.331\} & \{0.046, 0.112\} & \{0.874, 0.296\} & \{0.095, 0.312\} & \\
                                                   &  & &  & -26.0\% & 11.5\% & 88.9\% &  & & \\
\\
\hspace{3mm}Other Occupation                       & 2,000 & 450 & 29,500 & -0.007494 & -0.01866 & 0.02615* & 0.01104 & 0.008298 & -0.4977***  \\
                                                   &  & &  & (0.02871) & (0.02455) & (0.01452) & (0.03585) & (0.01879) & (0.169) \\
                                                   &  & &  & \{0.8919, 0.5117\} & \{0.06215, 0.3549\} & \{0.04595, 0.1334\} & \{0.8725, 0.364\} & \{0.06861, 0.1541\} & \\
                                                   &  & &  & -1.97\% & -6.37\% & 29.9\% & 2.17\% & 9.71\% & \\
\\
\hspace{3mm}US-Born                                & 2,700 & 500 & 40,500 & -0.03542* & 0.000687 & 0.03496*** & -0.03898 & 0.03245 & -0.6043***  \\
                                                   &  & &  & (0.02102) & (0.01946) & (0.01108) & (0.02495) & (0.0228) & (0.1544) \\
                                                   &  & &  & \{0.9212, 0.6176\} & \{0.04523, 0.34883\} & \{0.03357, 0.09002\} & \{0.9007, 0.4439\} & \{0.09464, 0.2121\} & \\
                                                   &  & &  & -11.7\% & 0.226\% & 61.9\% & -8.53\% & 27.6\% & \\
\\
\hspace{3mm}Foreign-Born                           & 1,400 & 500 & 21,500 & 0.01089 & -0.0292* & 0.01831 & 0.01766 & 0.00705 & -0.3238  \\
                                                   &  & &  & (0.02667) & (0.01579) & (0.02307) & (0.02812) & (0.02237) & (0.2575) \\
                                                   &  & &  & \{0.8898, 0.5695\} & \{0.05298, 0.2381\} & \{0.05722, 0.1924\} & \{0.8719, 0.3962\} & \{0.07259, 0.1886\} & \\
                                                   &  & &  & 3.40\% & -15.8\% & 13.5\% & 3.71\% & 6.08\% & \\
\\
\hline
\\
\\
\hline\hline
\end{tabular}

==> tables/regressions_dosage.tex <==


\begin{tabular}{lccccccccccccccccccc} \hline\hline
& (1) & (2) & (3) & & (4) & (5) & (6) & & (7) & (8) & (9) & & (10) & (11) & (12) & & (13) & (14) & (15) \\
\hline
\hline
\\
\\
\textbf{Panel A: Single-R01 Labs} \\
\hline
& \multicolumn{3}{c}{Univ.} & & \multicolumn{3}{c}{Industry} & & \multicolumn{3}{c}{No Admin.} & & \multicolumn{3}{c}{IHS Earnings} & & \multicolumn{3}{c}{IHS Earnings (Fully Attached)} \\
\hline
\\
\hspace{3mm}Full Sample                            & -0.02104 & -0.02344 & -0.0192 &  & -0.009197 & 0.01253 & -0.02589 & & 0.03024*** & 0.01091 & 0.0451*** & & -0.5228*** & -0.3079* & -0.6879*** & & -0.2268*** & -0.1952*** & -0.2534***\\
                                                   & (0.01843) & (0.02712) & (0.02323) &  & (0.0147) & (0.01692) & (0.02278) & & (0.01168) & (0.01494) & (0.016) & & (0.01373) & (0.1824) & (0.1825) & & (0.06271) & (0.06838) & (0.08843)\\
                                                   & \multicolumn{3}{c}{\{0.9101, 0.6023\}} &  & \multicolumn{3}{c}{\{0.048, 0.2751\}} & &  \multicolumn{3}{c}{\{0.0419, 0.1226\}} \\
                                                   & -6.84\% & -7.62\% & 6.24\% &  & -4.05\% & -5.52\% & -11.4\% & & 37.5\% & 13.5\% & 55.9\%\\
\\

\\
\hline
\\
\\
\hline
30 Day (Baseline)  &  $\times$ &  & & &  $\times$ &  & & & $\times$ & & & & $\times$ & & & & $\times$\\
90+ Days (High Dose)  &     &  $\times$ & & &   & $\times$  & & & &  $\times$ & & & & $\times$ & & & & $\times$ \\
30-90 Days (Low Dose)  &     &  & $\times$  & &  & & $\times$ & & & &  $\times$ & & &  & $\times$ & & & & $\times$\\
\hline\hline
\end{tabular}

==> tables/regressions_earnings.tex <==


\begin{tabular}{lccccccccccccccccccc} \hline\hline
& (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
\hline
\hline
\\
\\
\textbf{Panel A: Multiple-R01 Labs} \\
\hline
& Full Sample & Faculty & Post-Doc/Grad & Post-Doc & Grad & Other & US-Born & Foreign-Born \\
\hline
\\
No Attachment Restriction                       & 0.04929 \\
                                                & (0.0965) \\
\hspace{3mm}Personnel                           & 13,500 \\
\hspace{3mm}R01s                                & 1,200 \\
\hspace{3mm}Observations                        & 229,000 \\
\\         
Partially Attached                              & 0.05619 \\
                                                & (0.07265) \\
\hspace{3mm}Personnel                           & 13,000 \\
\hspace{3mm}R01s                                & 1,200 \\
\hspace{3mm}Observations                        & 214,000 \\
\\
Fully Attached                                  & -0.05888* \\
                                                & (0.03538)   \\
\hspace{3mm}Personnel                           & 11,000 \\
\hspace{3mm}R01s                                & 1,200 \\
\hspace{3mm}Observations                        & 183,000 \\
\hline
\\
\\
\textbf{Panel B: Single-R01 Labs} \\
\hline
& Full Sample & Faculty & Post-Doc/Grad & Post-Doc & Grad & Other & US-Born & Foreign-Born \\
\hline
\\
No Attachment Restriction                & -0.5228*** & -0.1377 & -0.7426*** & -0.8227 & -0.7494*** & -0.4977*** & -0.6043*** & -0.3238 \\
                                         & (0.1373) & (0.1556) & (0.2772) & (0.5213) & (0.2505) & (0.169) & (0.1544) & (0.2575) \\
\hspace{3mm}Personnel                    & 4,200 & 900 & 1,300 & 550 & 750 & 2,000 & 2,700 & 1400 \\
\hspace{3mm}R01s                         & 600 & 500 & 400 & 250 & 300 & 450 & 500 & 500 \\
\hspace{3mm}Observations                 & 61,500 & 14,000 & 18,500 & 7,500 & 11,000 & 29,500 & 40,500 & 21,500 \\                                                  
\\
Partially Attached                       & -0.3627***  \\
                                         & (0.1244)  \\
\hspace{3mm}Personnel                    & 4,000  \\
\hspace{3mm}R01s                         & 600  \\
 \hspace{3mm}Observations                & 58,500 \\                                               
\\
Fully Attached                           & -0.2268*** & -0.04708 & -0.2154 & -0.1559 & -0.1342 & -0.4021  \\
                                         & (0.06271) & (0.0891) & (0.1308) & (0.1122) & (0.1076) & (0.1765)  \\
\hspace{3mm}Personnel                    & 3,400 & 850 & 950 & & & 1,600 \\
\hspace{3mm}R01s                         & 600 & 500 & 350 & & & 450 \\                                               
\hspace{3mm}Observations                 & 49,500 & 13,500 & 13,500 & & & 23,000\\   
\\
\hline
\\
\\
\hline\hline
\end{tabular}

==> tables/regressions_iv_resubs.tex <==


\begin{tabular}{lccccccccccccccccccc} \hline\hline
& (1) & (2) & (3) & & (4) & (5) & (6) & & (7) & (8) & (9) & & (10) & (11) & (12) & & (13) & (14) & (15) \\
\hline
\hline
\\
\\
\textbf{Panel A: Multiple-R01 Labs} \\
\hline
& \multicolumn{3}{c}{Univ.} & & \multicolumn{3}{c}{Industry} & & \multicolumn{3}{c}{No Admin.} & & \multicolumn{3}{c}{IHS Earnings} & & \multicolumn{3}{c}{IHS Earnings (Fully Attached)} \\
\hline
\\
\hspace{3mm}Full Sample                            & 0.005576 & 0.003286 & -0.03126 &  & 0.003727 & -0.00106 & 0.03846 & & -0.009303 & -0.00223 & -0.007194 & & 0.04929 & -0.01742 & 0.2171 & & -0.05888* & -0.0533 \\
                                                   & (0.01325) & (0.01449) & (0.02338) &  & (0.01009) & (0.01109) & (0.01884) & & (0.008569) & (0.00868) & (0.02241) & & (0.0965) & (0.09382) & (0.2857) & & (0.03538) & (0.03431) \\
                                                   & \multicolumn{3}{c}{\{0.9137, 0.5750\}} &  & \multicolumn{3}{c}{\{0.0356, 0.2688\}} & &  \multicolumn{3}{c}{\{0.0507, 0.1562\}} \\
                                                   & 1.65\% & 0.97\% & -9.23\% &  & 1.60\% & -0.45\% & 16.49\% & & -8.82\% & -2.11\% & -6.82\%\\
\\
\\
\textbf{Panel B: Single-R01 Labs} \\
\hline
& \multicolumn{3}{c}{Univ.} & & \multicolumn{3}{c}{Industry} & & \multicolumn{3}{c}{No Admin.} & & \multicolumn{3}{c}{IHS Earnings} & & \multicolumn{3}{c}{IHS Earnings (Fully Attached)} \\
\hline
\\
\hspace{3mm}Full Sample                            & -0.02104 & -0.02231 & 0.01897 &  & -0.009197 & -0.009729 & -0.03395 & & 0.03024*** & 0.03204*** & 0.01498 & & -0.5228*** & -0.5035*** & -0.2817 & & -0.2268*** & -0.1792*** \\
                                                   & (0.01843) & (0.02024) & (0.04559) &  & (0.0147) & (0.01796) & (0.03241) & & (0.01168) & (0.01068) & (0.0302) & & (0.01373) & (0.1235) & (0.4161) & & (0.06271) & (0.06271) \\
                                                   & \multicolumn{3}{c}{\{0.9101, 0.6023\}} &  & \multicolumn{3}{c}{\{0.048, 0.2751\}} & &  \multicolumn{3}{c}{\{0.0419, 0.1226\}} \\
                                                   & -6.84\% & -7.52\% & 6.16\% &  & -4.05\% & -4.28\% & -14.95\% & & 37.5\% & 39.7\% & 18.6\%\\
\\

\\
\hline
\\
\\
\hline
C-S ATT  &  $\times$ &  & & &  $\times$ &  & & & $\times$ & & & & $\times$ & & & & $\times$\\
C-S ATT Resub. Cov.  &     &  $\times$ & & &   & $\times$  & & & &  $\times$ & & & & $\times$ & & & & $\times$ \\
IV  &     &  & $\times$  & &  & & $\times$ & & & &  $\times$ & & &  & $\times$ & & & & $\times$\\
\hline\hline
\end{tabular}

==> tables/regressions_noadmin.tex <==


\begin{tabular}{lccccccccccccccccccc} \hline\hline
& (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline
\hline
\\
\\
\textbf{Panel A: Single-R01 Labs} \\
\hline
& Personnel & R01s & Obs. & No Admin. & No Admin. & No Admin. & No Admin. & No Admin. & No Admin. & No Admin.  & No Admin. & No Admin.  & In Census (DID) \\
&  & & &  & In 2020 & Not In 2020 & Pubs & No Pubs & In 2020 & In 2020 & Not In 2020 & Not In 2020 & 2000/2010/2020 \\
&  &  &  &  &  & & &  & Pubs & No Pubs & Pubs & No Pubs \\
\hline
\\
\hspace{3mm}Full Sample                            & 4,200 & 600 & 61,500 & 0.03024*** & 0.01465 & 0.01559** & 0.004483 & 0.02586** & & & & & -0.02941**  \\
                                                   &  & &  & (0.01168) & (0.009575) & (0.006694) & (0.005851) & (0.009458) & & & & & (0.01487) \\
                                                   &  & &  & \{0.0419, 0.1226\} & \{0.02863, 0.06674\} & \{0.01327, 0.05586\} & \{0.00812, 0.03395\} & \{0.03378, 0.08865\} & \{0.005707, 0.01331\} & \{0.02292, 0.05343\} &  \{0.002413, 0.02064\} & \{0.01086, 0.03522\} \\
\\
\hspace{3mm}Faculty                                & 900 & 500 & 14,000 & 0.00302 & 0.006097 & -0.002078 & 0.01008 & -0.003775 & & & & & 0.04665 \\
                                                   &  & &  & (0.01523) & (0.01414) & (0.01766) & (0.0138) & (0.01237) & & & & & (0.03169) \\
                                                   &  & &  & \{0.008174, 0.04348\} &  &  &  & \\
\\
\hspace{3mm}Post-Doc/Grad Student                  & 1,300 & 400 & 18,500 & 0.06104*** & 0.01925 & 0.04315** & 0.00257 & 0.05868*** & & & & & -0.02337 \\
                                                   &  & &  & (0.02353) & (0.01776) & (0.01773) & (0.01324) & (0.02096) & & & & & (0.0393) \\
                                                   &  & &  & \{0.05979, 0.1585\} &  &  & &  \\
\\
\hspace{3mm}Other Occupation                       & 2,000 & 450 & 29,500 &  0.02615* & 0.01498 & 0.01143 & 0.006563 & 0.02032* & & & & & -0.04322* \\
                                                   &  & &  & (0.01452) & (0.01257) & (0.008268) & (0.007167) & (0.01233) & & & & & (0.02462) \\
                                                   &  & &  & \{0.04595, 0.1334\} &  &  &  &  \\
\\
\hspace{3mm}US-Born                                & 2,700 & 500 & 40,500 & 0.03496*** & 0.0262** & 0.01063** & 0.011* & 0.02525*** & 0.009127 & 0.01815** & 0.003393 & 0.008823* & -0.01572 \\
                                                   &  & &  & (0.01108) & (0.01138) & (0.00519) & (0.005925) & (0.009597) & (0.005595) & (0.008856) & (0.004069) & (0.005007) & (0.01828) \\
                                                   &  & &  & \{0.03357, 0.09002\} & \{0.028442, 0.07576\} & \{0.005128, 0.01426\} & \{0.00513, 0.01961\} & \{0.02844, 0.07041\} \\
\\
\hspace{3mm}Foreign-Born                           & 1,400 & 500 & 21,500 & 0.01831 & -0.008865 & 0.0282 & -0.006551 & 0.02472 & 0.0009497 & -0.00977 & -0.007738 & 0.0357** & -0.03897 \\
                                                   &  & &  & (0.02307) & (0.01274) & (0.01844) &(0.01144) & (0.01844) & (0.006306) & (0.01159) & (0.01156) & (0.01725) & (0.03973) \\
                                                   &  & &  & \{0.05722, 0.1924\} & \{0.02904, 0.0476\} & \{0.02818, 0.1448\} & \{0.01367, 0.0648\} & \{0.04355, 0.1276\} \\
\\
\hline
\\
\\
\hline\hline
\end{tabular}

==> tables/regressions_noadmin_percents.tex <==


\begin{tabular}{lccccccccccccccccccc} \hline\hline
& (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
\hline
\hline
\\
\\
\textbf{Panel A: Multiple-R01 Labs} \\
\hline
& Full Sample & Faculty & Post-Doc/Grad & Post-Doc & Grad & Other & US-Born & Foreign-Born \\
\hline
\\
\hline
\\
\\
\textbf{Panel B: Single-R01 Labs} \\
\hline
& Full Sample & Faculty & Post-Doc/Grad & Post-Doc & Grad & Other & US-Born & Foreign-Born \\
\hline
\\
No Admin.                                & 0.03024*** & 0.00302 & 0.06104*** & 0.07513* & 0.05865*** & 0.02615* & 0.03496*** & 0.01831 \\                                         
\\
In 2020                                  & 0.01465 (48.4\%) & 0.006097 (152\%) & 0.01925 (30.8\%) & & &  0.01498 (56.7\%) & 0.0262** (71.1\%) & -0.008865 (-45.8\%)\\
Not In 2020                              & 0.01559** (51.6\%) & -0.002078 (-52\%) & 0.04315** (69.2\%) & & & 0.01143 (43.3\%) & 0.01063** (28.9\%) & 0.0282 (145.8\%) \\
\textit{Sum}                             & 0.03024 & 0.004019 & 0.0624 & & & 0.02641 & 0.03683 & 0.019335\\                          
\\
\\
Publications                             & 0.004483 (14.8\%) & 0.01008 (159.9\%) & 0.00257 (4.2\%) & & & 0.006563 (24.4\%) & 0.011* (30.3\%) & -0.006551 (-36.1\%) \\
No Publications                          & 0.02586** (85.2\%) & -0.003775 (-59.9\%) & 0.05868*** (95.8\%) & & & 0.02032* (75.6\%) & 0.02525*** (69.7\%) & 0.02472 (136.1\%) \\
\textit{Sum}                             & 0.030343  & 0.006305 & 0.06125 & & & 0.026883 & 0.03625 & 0.018169 \\
\\
In 2020, Publications                    &  & & & & & &  0.009127 (33.5\%) & 0.0009497 (-10.8\%) \\
In 2020, No Publications                 &  & & & & & & 0.01815** (66.5\%) & -0.00977 (110.8\%) \\
\textit{Sum}                             &  & & & & & & 0.027277 &  -0.0088203 \\
\\
Not In 2020, Publications                &  & & & & & &  0.003393 (27.8\%) & -0.007738 (-27.7\%) \\
Not In 2020, No Publications             &  & & & & & &  0.008823* (72.2\%) & 0.0357** (127.7\%) \\
\textit{Sum}                             &  & & & & & &  0.012216 & 0.027962  
\\
\hline
\\
\\
\hline\hline
\end{tabular}
